An Efficient and Balanced Graph Partition Algorithm for the Subgraph-Centric Programming Model on Large-scale Power-law Graphs

The subgraph-centric programming model is a promising approach and has been applied in many state-of-the-art distributed graph computing frameworks. However, traditional graph partition algorithms have significant difficulties in processing large-scale power-law graphs. The major problem is the communication bottleneck found in many subgraph-centric frameworks. Detailed analysis indicates that the communication bottleneck is caused by the huge communication volume or the extreme message imbalance among partitioned subgraphs. The traditional partition algorithms do not consider both factors at the same time, especially on power-law graphs. In this paper, we propose a novel efficient and balanced vertex-cut graph partition algorithm (EBV) which grants appropriate weights to the overall communication cost and communication balance. We observe that the number of replicated vertices and the balance of edge and vertex assignment have a great influence on communication patterns of distributed subgraph-centric frameworks, which further affect the overall performance. Based on this insight, We design an evaluation function that quantifies the proportion of replicated vertices and the balance of edges and vertices assignments as important parameters. Besides, we sort the order of edge processing by the sum of end-vertices' degrees from small to large. Experiments show that EBV reduces replication factor and communication by at least 21.8% and 23.7% respectively than other self-based partition algorithms. When deployed in the subgraph-centric framework, it reduces the running time on power-law graphs by an average of 16.8% compared with the state-of-the-art partition algorithm. Our results indicate that EBV has a great potential in improving the performance of subgraph-centric frameworks for the parallel large-scale power-law graph processing.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> preliminaries.tex <==
\section{Preliminaries}\label{sec:pre}
In this section, we introduce some notations and metrics for the rest of this paper.

Let $G = (V, E)$ be a directed graph, where $V$ denotes the set of vertices and $E$ denotes the set of edges. 
An edge is represented as a pair of vertices $(u, v)$ where $u$ is the source vertex and $v$ is the target vertex.
For the undirected graph, we replace each undirected edge with two edges with opposite directions.
Suppose we partition the graph $G$ into $p$ subgraphs, we denote $G_i(V_i, E_i)$, $i \in [1, p]$ as the $i^{th}$ subgraph.

For the vertex-cut (edge partitioning) algorithms, they partition the edge set $E$ into $p$ subsets.
Let $E_1 \cup E_2 \cup \cdots \cup E_p = E$ be the $p$ partitions of $E$, i.e. $E_i \cap E_j = \emptyset$, $\forall i \ne j$. 
%The corresponding subgraph is represented as $G_i(V_i, E_i)$. 
Here we define $V_i = \{u |(u, v) \in E_i \lor (v, u) \in E_i \}$ as the set of vertices covered by $E_i$. 
Due to the definition of $V_i$, there may exist some replicated vertices which have the same vertex ID but belong to different subgraphs.
%For the sake of convenience, we remark the vertex $u \in V_{m_i}$ as $u_{m_i}$.

For the edge-cut (vertex partitioning) algorithms, they partition the vertex set $V$.
Let $V_1 \cup V_2 \cup \cdots \cup V_p = V$ and $V_i \cap V_j = \emptyset$ for all $i \ne j$, we define $E_i = \{(u, v) | u \in V_i \lor v \in V_i \}$. The definition of $E_i$ here means that there exist some replicated edges such that $E_i \cap E_j \ne \emptyset$.

Further, we introduce three metrics: edge imbalance factor, vertex imbalance factor and replication factor.
The edge imbalance factor is defined as  
\begin{math}
\frac{\max_{i=1,...,p} |E_{i}|}{|E|/p}
\end{math} 
, while the vertex imbalance factor is defined as 
\begin{math}
\frac{\max_{i=1,...,p} |V_{i}|}{\sum_{i=1}^{p} |V_{i}|/p}
\end{math}
. Both of them are used to measure the balance of partition results.

For the vertex-cut algorithm, the replication factor is defined as   
\begin{math}
\frac{\sum_{i=1}^{p} |V_{i}|}{|V|}
\end{math}.
However, we have $\sum_{i=1}^{p} |V_{i}| = |V|$ for the edge-cut algorithm.
Thus the definition of the replication factor cannot be directly adapted and we define 
\begin{math}
\frac{\sum_{i=1}^{p} |E_{i}|}{|E|}
\end{math} as the replication factor for the edge-cut algorithm.
The replication factor represents the average number of replicas for a vertex or edge.

For the three metrics above, the closer they are to 1, the better the performance they represent.
These metrics are also widely used in~\cite{boman2013scalable,chen2019powerlyra,xie2014distributed, ne}.

%However, we cannot measure the imbalance of partitioned results only by the edge imbalance factor. Considering two subgraphs $G_i(V_i, E_i)$ and $G_j(V_j, E_j)$ that $|E_i| = |E_j|$ but $|V_i| \ne |V_j|$. Although the edge imbalance factor of them is $1$, the complexities of many graph algorithms on them are different. (Usually, the complexity of a graph algorithm is related to the number of vertices.) Thus we propose the vertex imbalance factor.

%Notice that $\sum_{i=1}^{p} |E_{i}| = |E|$, thus the corresponding edge replication factor $\frac{\sum_{i=1}^{p} |E_{i}|}{|E|}$ is always $1$ and meaningless. 
